Genetic Algorithms for Lens Design: a Review

Genetic algorithms (GAs) have a long history of over four decades. GAs are adaptive heuristic search algorithms that provide solutions for optimization and search problems. The GA derives expression from the biological terminology of natural selection, crossover, and mutation. In fact, GAs simulate the processes of natural evolution. Due to their unique simplicity, GAs are applied to the search space to find optimal solutions to various problems in science and engineering. Using GAs for lens design was investigated mostly in the 1990s, but were not fully exploited. But in the past few years there have been a number of newer studies exploring the application of GAs or hybrid GAs in optical design. In this paper we discuss the basic ideas behind GAs and demonstrate their application in optical lens design.

==> files/copyright.tex <==
% University Assignment Title Page 
% LaTeX Template
% Version 1.0 (27/12/12)
%
% This template has been downloaded from:
% http://www.LaTeXTemplates.com
%
% Original author:
% WikiBooks (http://en.wikibooks.org/wiki/LaTeX/Title_Creation)
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
% 
% Instructions for using this template:
% This title page is capable of being compiled as is. This is not useful for 
% including it in another document. To do this, you have two options: 
%
% 1) Copy/paste everything between \begin{document} and \end{document} 
% starting at \begin{titlepage} and paste this into another LaTeX file where you 
% want your title page.
% OR
% 2) Remove everything outside the \begin{titlepage} and \end{titlepage} and 
% move this file to the same directory as the LaTeX file you wish to add it to. 
% Then add \input{./title_page_1.tex} to your LaTeX file where you want your
% title page.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\title{Title page with logo}
%----------------------------------------------------------------------------------------
%	PACKAGES AND OTHER DOCUMENT CONFIGURATIONS
%-------------------------------------------

==> files/framebox1.tex <==
\colorlet{framecolor}{black} %VioletRed4
\setlength\FrameRule{0pt}
{\small
\begin{frshaded*}
	\begin{itemize}
	\item \textbf{Chromosome} (= genotype): often as binary strings, more precisely a number of parameters which determine a solution and belong to a problem solved by the GA \cite{wiki2016chromosome}
  	%\item \textbf{Genes:}
	%\item \textbf{Genome:}
	\item \textbf{Phenotype:} genotype with mental properties, coding scheme to represent the chromosomes
	\item \textbf{Population:} set of all chromosomes
    \item \textbf{Fitness (function):} feedback to GA to find a solution. A value which is related to a chromosome \cite{chen1997experiment}.
    \item \textbf{Gene set:} a number or population of candidate solutions
	\item \textbf{GA:} optimization algorithm and stochastic search methods for populations influenced by natural processes to solve optimization problems by applying a population of solutions
    \item \textbf{Merit function:}    
  	\end{itemize}
%\vspace{20pt}
\end{frshaded*}
}
